UniAPO: Unified Multimodal Automated Prompt Optimization

Prompting is fundamental to unlocking the full potential of large language models. To automate and enhance this process, automatic prompt optimization (APO) has been developed, demonstrating effectiveness primarily in text-only input scenarios. However, extending existing APO methods to multimodal tasks, such as video-language generation introduces two core challenges: (i) visual token inflation, where long visual token sequences restrict context capacity and result in insufficient feedback signals; (ii) a lack of process-level supervision, as existing methods focus on outcome-level supervision and overlook intermediate supervision, limiting prompt optimization. We present UniAPO: Unified Multimodal Automated Prompt Optimization, the first framework tailored for multimodal APO. UniAPO adopts an EM-inspired optimization process that decouples feedback modeling and prompt refinement, making the optimization more stable and goal-driven. To further address the aforementioned challenges, we introduce a short-long term memory mechanism: historical feedback mitigates context limitations, while historical prompts provide directional guidance for effective prompt optimization. UniAPO achieves consistent gains across text, image, and video benchmarks, establishing a unified framework for efficient and transferable prompt optimization.

==> sec/6.checklist.tex <==
\makeatletter
\@ifundefined{isChecklistMainFile}{
  % We are compiling a standalone document
  \newif\ifreproStandalone
  \reproStandalonetrue
}{
  % We are being \input into the main paper
  \newif\ifreproStandalone
  \reproStandalonefalse
}
\makeatother

\ifreproStandalone
\setlength{\pdfpagewidth}{8.5in}
\setlength{\pdfpageheight}{11in}
\frenchspacing

\fi
\setlength{\leftmargini}{20pt}
\makeatletter\def\@listi{\leftmargin\leftmargini \topsep .5em \parsep .5em \itemsep .5em}
\def\@listii{\leftmargin\leftmarginii \labelwidth\leftmarginii \advance\labelwidth-\labelsep \topsep .4em \parsep .4em \itemsep .4em}
\def\@listiii{\leftmargin\leftmarginiii \labelwidth\leftmarginiii \advance\labelwidth-\labelsep \topsep .4em \parsep .4em \itemsep .4em}\makeatother

\setcounter{secnumdepth}{0}
\renewcommand\thesubsection{\arabic{subsection}}
\renewcommand\labelenumi{\thesubsection.\arabic{enumi}}

\newcounter{checksubsection}
\newcounter{checkitem}[checksubsection]

\newcommand{\checksubsection}[1]{%
  \refstepcounter{checksubsection}%
  \paragraph{\arabic{checksubsection}. #1}%
  \setcounter{checkitem}{0}%
}

\newcommand{\checkitem}{%
  \refstepcounter{checkitem}%
  \item[\arabic{checksubsection}.\arabic{checkitem}.]%
}
\newcommand{\question}[2]{\normalcolor\checkitem #1 #2 \color{blue}}
\newcommand{\ifyespoints}[1]{\makebox[0pt][l]{\hspace{-15pt}\normalcolor #1}}

\section*{Reproducibility Checklist}

\noindent

\checksubsection{General Paper Structure}
\begin{itemize}

\question{Includes a conceptual outline and/or pseudocode description of AI methods introduced}{(yes/partial/no/NA)}
yes

\question{Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results}{(yes/no)}
yes

\question{Provides well-marked pedagogical references for less-familiar readers to gain background necessary to replicate the paper}{(yes/no)}
yes

\end{itemize}
\checksubsection{Theoretical Contributions}
\begin{itemize}

\question{Does this paper make theoretical contributions?}{(yes/no)}
yes

	\ifyespoints{\vspace{1.2em}If yes, please address the following points:}
        \begin{itemize}
	
	\question{All assumptions and restrictions are stated clearly and formally}{(yes/partial/no)}
	yes

	\question{All novel claims are stated formally (e.g., in theorem statements)}{(yes/partial/no)}
	partial

	\question{Proofs of all novel claims are included}{(yes/partial/no)}
	yes

	\question{Proof sketches or intuitions are given for complex and/or novel results}{(yes/partial/no)}
	yes

	\question{Appropriate citations to theoretical tools used are given}{(yes/partial/no)}
	yes

	\question{All theoretical claims are demonstrated empirically to hold}{(yes/partial/no/NA)}
	yes

	\question{All experimental code used to eliminate or disprove claims is included}{(yes/no/NA)}
	yes
	
	\end{itemize}
\end{itemize}

\checksubsection{Dataset Usage}
\begin{itemize}

\question{Does this paper rely on one or more datasets?}{(yes/no)}
yes

\ifyespoints{If yes, please address the following points:}
\begin{itemize}

	\question{A motivation is given for why the experiments are conducted on the selected datasets}{(yes/partial/no/NA)}
	yes

	\question{All novel datasets introduced in this paper are included in a data appendix}{(yes/partial/no/NA)}
	yes

	\question{All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes}{(yes/partial/no/NA)}
	yes

	\question{All datasets drawn from the existing literature (potentially including authors' own previously published work) are accompanied by appropriate citations}{(yes/no/NA)}
	yes

	\question{All datasets drawn from the existing literature (potentially including authors' own previously published work) are publicly available}{(yes/partial/no/NA)}
	yes

	\question{All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing}{(yes/partial/no/NA)}
	yes

\end{itemize}
\end{itemize}

\checksubsection{Computational Experiments}
\begin{itemize}

\question{Does this paper include computational experiments?}{(yes/no)}
yes

\ifyespoints{If yes, please address the following points:}
\begin{itemize}

	\question{This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting}{(yes/partial/no/NA)}
	yes

	\question{Any code required for pre-processing data is included in the appendix}{(yes/partial/no)}
	no

	\question{All source code required for conducting and analyzing the experiments is included in a code appendix}{(yes/partial/no)}
	no

	\question{All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes}{(yes/partial/no)}
	yes
        
	\question{All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from}{(yes/partial/no)}
	yes

	\question{If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results}{(yes/partial/no/NA)}
	yes

	\question{This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks}{(yes/partial/no)}
	yes

	\question{This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics}{(yes/partial/no)}
	yes

	\question{This paper states the number of algorithm runs used to compute each reported result}{(yes/no)}
	yes

	\question{Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information}{(yes/no)}
	yes

	\question{The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank)}{(yes/partial/no)}
	partial

	\question{This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments}{(yes/partial/no/NA)}
	yes


\end{itemize}
\end{itemize}
\ifreproStandalone
\fi

==> sec/case/beauty/ERM/Initial_prompt.tex <==
\begin{tcolorbox}[breakable,
title=Initial Prompt,
colback=white,          % <-- 核心：设置背景为白色
colframe=black,         % <-- 设置黑色边框以保证可见性
coltext=black,          % 设置正文文字为黑色
% coltitle=black,         % 设置标题文字为黑色
% fonttitle=\bfseries,
]
\begin{lstlisting}
Keywords about beauty.
\end{lstlisting}
\end{tcolorbox}

==> sec/case/beauty/ERM/feedback.tex <==
\begin{tcolorbox}[breakable,
title=Generated Feedback,
colback=white,          % <-- 核心：设置背景为白色
colframe=black,         % <-- 设置黑色边框以保证可见性
coltext=black,          % 设置正文文字为黑色
% coltitle=black,         % 设置标题文字为黑色
% fonttitle=\bfseries,
]
\begin{lstlisting}
**Regulation #1: Prioritize keyword extraction based on visual cues from video frames**  

The extraction process must focus on identifying actionable keywords directly tied to visual elements in the video. For example, objects like makeup tools (e.g., eyelash curler, lip tint, perfume bottles) or actions (e.g., applying makeup, spraying perfume) should be prioritized as keywords. This regulation ensures that the visual content of the video frames is the primary source for keyword extraction, reducing reliance on less relevant text-based information. Additionally, extracted keywords should be validated against the policy to ensure they align with the intended context (e.g., beauty-related terms). 


**Regulation #2: Incorporate Visual Context Analysis for Implicit Keywords**

- Enhance the extraction process to integrate visual cues from the video frames. For example, if a product name or branding is prominently displayed in the video (e.g., "Shooting Stars Body Lotion" in Case #4), it should be included in the extracted keywords, even if it is not explicitly mentioned in the OCR or ASR. 

- Use the visual content to infer implicit keywords related to the policy theme (e.g., "Beauty Effect Display" in Case #3). This ensures the extraction captures the broader context and intent of the video content.
\end{lstlisting}
\end{tcolorbox}

==> sec/case/beauty/ERM/optimized_prompt.tex <==
\begin{tcolorbox}[breakable,
title=Optimized Prompt,
colback=white,          % <-- 核心：设置背景为白色
colframe=black,         % <-- 设置黑色边框以保证可见性
coltext=black,          % 设置正文文字为黑色
% coltitle=black,         % 设置标题文字为黑色
% fonttitle=\bfseries,
]
\begin{lstlisting}
1. **Objective**:  
   Extract beauty-related keywords from short videos using a zero-shot approach that integrates multimodal data (title, stickers, OCR, ASR, video frames). Ensure extracted keywords are specific, actionable, relevant, and aligned with the beauty theme.

2. **Multimodal Data Integration**:  
   - **Title and Stickers**:  
     Analyze video titles and sticker texts for explicit mentions of beauty-related terms, focusing on beauty products, techniques, or attributes (e.g., "glow serum," "natural makeup").  
   - **OCR (Optical Character Recognition)**:  
     Extract text from video frames to identify beauty-related keywords, such as product names, brand logos, or descriptive terms (e.g., "hydrating serum," "natural glow").  
   - **ASR (Automatic Speech Recognition)**:  
     Analyze spoken content to identify beauty-related concepts (e.g., "makeup tutorial," "skincare routine") and prioritize frequently mentioned or emphasized words.  
   - **Video Frames (Visual Context)**:  
     Perform a detailed visual analysis of objects, brand logos, or actions associated with beauty (e.g., lipstick application, facial cleansing). Infer implicit keywords from visual cues, even if absent in OCR or ASR.

3. **Regulations for Keyword Extraction**:  
   - **Regulation #1: Incorporate Visual Context Analysis for Implicit Keywords**:  
     - Identify implicit beauty-related terms through detailed visual content analysis (e.g., "lip tattoo application" or "Beauty Effect Display").  
     - Derive broader themes from visual context (e.g., "makeup transformation" if a step-by-step transformation is shown).  
     - Use surrounding objects and actions (e.g., facial cleansing routine) to infer related terms while ensuring relevance to beauty.  
   - **Regulation #2: Cross-Reference Modalities for Policy-Relevant Keywords**:  
     - Actively cross-reference ASR, OCR, and video frames to identify beauty-related terms.  
     - Weight keywords based on frequency and prominence (e.g., repeated ASR mentions or visually highlighted text in frames).  
   - **Regulation #3: Prioritize Visual Cues for Actionable Keywords**:  
     - Focus on actionable keywords tied to visual elements (e.g., tools like "makeup brush," actions like "applying foundation").  
     - Validate extracted keywords for alignment with the beauty theme and disregard irrelevant or ambiguous terms.  

4. **Handling Challenging or Noisy Examples**:  
   - **Noisy or Missing Data**:  
     - Prioritize reliable modalities (e.g., video frames, ASR) if specific modalities (e.g., OCR) are noisy or missing.  
     - Use contextual inference to fill gaps. For example, if ASR mentions "hydration" and frames show a lotion bottle, infer terms like "hydrating serum."  
   - **Visually Ambiguous Content**:  
     - Cross-reference textual data (title, stickers, OCR, ASR) to resolve ambiguities. If ambiguity persists, extract generic beauty-related terms (e.g., "beauty product," "makeup technique") based on the overall video context.  
   - **Contextual Inference**:  
     - Leverage evaluation descriptions and surrounding elements to infer keywords. For example, if frames depict a moisturizer alongside a facial routine, derive terms like "skincare routine" or "moisturizing cream."

5. **Keyword Prioritization Criteria**:  
   - **Frequency**: Keywords repeated in ASR or prominently displayed in visual elements (e.g., close-ups of product labels) take precedence.  
   - **Prominence**: Keywords visually emphasized (e.g., bold fonts, highlighted text) or audibly stressed are prioritized.  
   - **Relevance**: All extracted keywords must align with the beauty theme. Exclude irrelevant or off-topic terms (e.g., unrelated brand names, general phrases).

6. **Output Requirements**:  
   - The extracted keywords must be concise, specific, and presented as a list wrapped within `<answer>` and `</answer>` tags.  
   - Examples: `<answer>[lip gloss, hydrating serum, skincare routine]</answer>`.  
   - Avoid overly broad or vague terms.

7. **Verification and Validation**:  
   - **Quality Check**:  
     - Validate extracted keywords against the beauty policy to ensure alignment and adherence to the intended theme.  
     - Confirm that no critical visual or textual elements are overlooked.  
   - **Feedback Integration**:  
     - For videos with noisy or missing data, ensure that inferred keywords are derived logically using the most reliable modalities and contextual clues.  
     - Incorporate implicit keywords by analyzing visual content and cross-referencing with evaluation descriptions.

8. **Refinements Based on Feedback**:  
   - **Strengthened Multimodal Integration**:  
     - For missing or noisy OCR/ASR data, rely on video frames and evaluation descriptions (if available) to infer keywords. For example, if ASR mentions "makeup brands" and frames show recognizable logos, extract terms like "local makeup brands" or "vegan-certified cosmetics."  
   - **Enhanced Visual Context Analysis**:  
     - Extract implicit keywords by interpreting visual content. For instance, if a product is applied to the face, infer terms like "hydrating serum" or "foundation application."  
     - Use surrounding objects and actions to enhance understanding. For example, if a video shows a facial cleansing routine, infer "cleansing foam" or "skincare routine."  
     - Validate implicit keywords against evaluation descriptions. For example, if "radiance" is mentioned and frames show highlighters, include terms like "radiance booster."  

9. **Handling Feedback-Driven Challenges**:  
   - **Implicit Keyword Extraction**:  
     - Perform detailed visual analysis to infer implicit beauty-related terms, such as specific procedures (e.g., "eyelash extension"), tools (e.g., "tweezers," "sponges"), or outcomes (e.g., "dewy finish").  
   - **Broader Beauty Themes**:  
     - Derive broader beauty-related themes from visual narratives (e.g., "beauty tutorial").  
   - **Prioritization of Actionable Visual Elements**:  
     - Emphasize actionable keywords tied directly to visual elements (e.g., "blush application," "contouring brush").  
     - Validate inferred keywords against the overall visual and multimodal narrative to ensure consistency and relevance.
\end{lstlisting}
\end{tcolorbox}

==> sec/case/beauty/EvolPrompt/Initial_prompt.tex <==
\begin{tcolorbox}[breakable,
title=Initial Prompt,
colback=white,          % <-- 核心：设置背景为白色
colframe=black,         % <-- 设置黑色边框以保证可见性
coltext=black,          % 设置正文文字为黑色
% coltitle=black,         % 设置标题文字为黑色
% fonttitle=\bfseries,
]
\begin{lstlisting}
Keywords about beauty.
\end{lstlisting}
\end{tcolorbox}

==> sec/case/beauty/EvolPrompt/optimized_prompt.tex <==
\begin{tcolorbox}[breakable,
title=Optimized Prompt,
colback=white,          % <-- 核心：设置背景为白色
colframe=black,         % <-- 设置黑色边框以保证可见性
coltext=black,          % 设置正文文字为黑色
% coltitle=black,         % 设置标题文字为黑色
% fonttitle=\bfseries,
]
\begin{lstlisting}
Generate n keywords related to beauty that encapsulate its diverse aspects, such as physical, emotional, cultural, and artistic dimensions.
\end{lstlisting}
\end{tcolorbox}

==> sec/case/beauty/UniAPO/Initial_prompt.tex <==
\begin{tcolorbox}[breakable,
title=Initial Prompt,
colback=white,          % <-- 核心：设置背景为白色
colframe=black,         % <-- 设置黑色边框以保证可见性
coltext=black,          % 设置正文文字为黑色
% coltitle=black,         % 设置标题文字为黑色
% fonttitle=\bfseries,
]
\begin{lstlisting}
Keywords about beauty.
\end{lstlisting}
\end{tcolorbox}

==> sec/case/beauty/UniAPO/cold_start_case_prompt.tex <==
\begin{tcolorbox}[breakable,
title=Input Prompt,
colback=white,          % <-- 核心：设置背景为白色
colframe=black,         % <-- 设置黑色边框以保证可见性
coltext=black,          % 设置正文文字为黑色
% coltitle=black,         % 设置标题文字为黑色
% fonttitle=\bfseries,
]
\begin{lstlisting}
The keyword extractor must identify and extract concise, relevant, and contextually accurate keywords specifically related to sports from the provided video. The assessment must consider the following components:  

1. \textbf{Title}: Analyze the title for any explicit mentions or implications of sports-related terms or activities.  
2. **Sticker Texts**: Evaluate text present in stickers within the video for sports-specific language or references.  
3. **OCR (Optical Character Recognition)**: Examine all visual text extracted from the video frames for keywords associated with sports, including sports names, terminologies, or related terms.  
4. **ASR (Automatic Speech Recognition)**: Process the spoken content within the video to identify sports-related mentions or themes.  
5. **Video Frames**: Contextually interpret visual elements in the frames (e.g., players, equipment, locations) to verify relevance to sports.  

The extracted keywords must be:  
- **Specific**: Pertinent to sports (e.g., "soccer," "basketball").  
- **Concise**: Avoiding redundancy or overly broad terms.  
- **Contextually Relevant**: Reflecting the actual theme or content presented in the video.  

Exclude generic or unrelated terms that do not directly relate to sports. Perform a holistic evaluation of all input components to ensure accurate keyword extraction. 
\end{lstlisting}
\end{tcolorbox}

==> sec/case/beauty/UniAPO/feedback.tex <==
\begin{tcolorbox}[breakable,
title=Generated Feedback,
colback=white,          % <-- 核心：设置背景为白色
colframe=black,         % <-- 设置黑色边框以保证可见性
coltext=black,          % 设置正文文字为黑色
% coltitle=black,         % 设置标题文字为黑色
% fonttitle=\bfseries,
]
\begin{lstlisting}
**Regulation #1: Prioritize Visual Frame Context for Implicit Keyword Inference**  

- Ensure that visual frames are thoroughly analyzed for implicit beauty-related processes, tools, or themes.  
- Introduce a systematic approach to identify recurring objects, tools, or actions across frames. For example:  
    - If frames consistently depict a skincare routine, infer keywords like "skincare tools" or "acne treatment."  
    - If frames show makeup application, extract keywords such as "makeup routine" or "post-surgery recovery."  
    - Cross-reference visual elements with other modalities to confirm or enhance inferred keywords. For instance, if ASR mentions "hydrating serum" and frames show a skincare demonstration, prioritize extracting "hydrating skincare routine."  
    - Emphasize contextually significant associations to avoid missing implicit keywords like "Beauty Process" or "Women\'s Eye Beauty."


**Regulation #2: Cross-Referencing Modalities for Consistent Keyword Identification**  

Enhance keyword extraction by cross-referencing visual frame data with video information (e.g., OCR and ASR outputs) to ensure consistency and accuracy. For example:  

    - If ASR mentions "long-lasting perfume" and frames display a branded perfume like "Ocean di Gioia," synthesize keywords such as "long-lasting fragrance" or "women\'s perfume."  

    - If OCR highlights "hydrating serum" and frames show a skincare product, extract keywords like "hydrating skincare routine" or "serum for luminous skin."  \n\nAdditionally, ensure recurring visual elements (e.g., tools, products, or processes) are consistently identified across frames. For example:  
        - If a specific tool or product appears repeatedly, extract keywords like "skincare tools" or "luxury fragrance collection."  

Prioritize clarity and avoid redundancy unless necessary to differentiate distinct aspects of the content (e.g., product types, attributes, or demonstrated techniques). This cross-referencing approach ensures comprehensive and contextually relevant keyword extraction.


**Regulation #3: Cross-Modal Synthesis for Enhanced Keyword Precision**

- Enhance the synthesis process by integrating visual frame analysis with ASR and OCR data. For example, if ASR mentions "V Beauty Ebony Foundation" and visual frames show the product, generate keywords like "V Beauty foundation" or "Ebony shade foundation."

- Prioritize alignment between modalities to ensure comprehensive keyword extraction. If a modality (e.g., ASR) provides detailed product descriptions, confirm these details with visual elements before including them as keywords.

- Address missing or ambiguous data by leveraging available modalities. For instance, if OCR data is incomplete, rely on ASR and visual frames to infer implicit keywords (e.g., "brightening tips" for a lotion product).

- Avoid redundancy by ensuring each keyword reflects a unique aspect of the content, unless repetition is necessary for contextual clarity.


\end{lstlisting}
\end{tcolorbox}

==> sec/case/beauty/UniAPO/optimized_prompt.tex <==
\begin{tcolorbox}[breakable,
title=Optimized Prompt,
colback=white,          % <-- 核心：设置背景为白色
colframe=black,         % <-- 设置黑色边框以保证可见性
coltext=black,          % 设置正文文字为黑色
% coltitle=black,         % 设置标题文字为黑色
% fonttitle=\bfseries,
]
\begin{lstlisting}
### Purpose:
The zero-shot keyword extraction model is designed to identify and extract precise, relevant keywords directly tied to beauty from short video content. It must analyze all provided components comprehensively, ensuring no critical details are overlooked. Extracted keywords must be concise, unambiguous, and specific to the beauty domain, avoiding irrelevant or overly generalized terms.

---

### Components for Keyword Extraction:
1. **Title**:
   - Evaluate the title for explicit or implied beauty-related keywords (e.g., skincare, makeup, hairstyles, fashion trends).
   - Avoid ambiguous or irrelevant terms that lack clear ties to the beauty domain.

2. **Stickers**:
   - Analyze sticker text for mentions of beauty-related themes, products, or practices.
   - Extract keywords directly tied to beauty-related contexts while ignoring unrelated or decorative sticker text.

3. **OCR (Optical Character Recognition)**:
   - Extract text from video frames for beauty-related keywords such as product names, brand mentions, or descriptive beauty terms (e.g., "hydrating serum," "lip gloss").
   - Prioritize OCR text that complements other components and directly supports the beauty theme.

4. **ASR (Automatic Speech Recognition)**:
   - Process spoken content for beauty-related terms, discussions, tips, or routines.
   - Extract keywords reflecting beauty-specific content, such as product recommendations, tutorials, or procedures, ensuring alignment with visual cues.

5. **Video Frames**:
   - Place the highest priority on analyzing visual elements within the video frames.
   - Extract keywords related to beauty products, tools, or processes shown. Examples include product packaging, brand labels, tools (e.g., guasha, eyelash curlers), and aesthetic visuals indicative of beauty themes.
   - Include both the product and the associated process for demonstrations (e.g., "guasha tool," "facial skincare routine").
   - Recognize promotional intent, such as "Beauty Advertisement."

---

### Keyword Extraction Principles:
1. **Prioritize Video Frame Analysis**:
   - Treat video frames as the primary source of evidence for extracting keywords.
   - Extract keywords that reflect visible beauty products, tools, or demonstrated processes in the frames.
   - Include both the product name and its category (e.g., "Charlotte Tilbury Lip Plumper," "lip plumper") for specificity and precision.

2. **Contextual Relevance**:
   - Ensure extracted keywords align with the beauty domain and are directly tied to the context provided by the video content.
   - Avoid overgeneralization or ambiguous terms unless explicitly supported by evidence from the video components.

3. **Specificity and Precision**:
   - Extract precise keywords referencing specific beauty products, tools, or routines.
   - Avoid overly broad terms unless explicitly justified by the content.

4. **Multimodal Integration**:
   - Systematically integrate insights from all components (title, stickers, OCR, ASR, and video frames).
   - Prioritize video frames but validate or enrich keywords using OCR and ASR data.
   - Cross-reference data across modalities to confirm accuracy and relevance. For example:
      - If ASR mentions "lip tint" and the video frames show the corresponding product, ensure the keyword reflects both modalities.
      - If video frames show "Mykonos snail extract face cream" and ASR mentions "hydrating cream," extract "Mykonos snail extract face cream with hydrating properties."

5. **Handling Ambiguous, Conflicting, or Missing Data**:
   - If a component lacks relevant content or is noisy, rely on other components to ensure accuracy.
   - Use visual cues from video frames to resolve conflicting or ambiguous data.
   - Avoid force-fitting unrelated keywords; if minimal beauty-related content exists, refrain from extracting irrelevant terms.

6. **Demonstrated Processes and Promotional Context**:
   - Reflect demonstrated processes in the extracted keywords (e.g., "lip tattoo procedure," "facial rejuvenation").
   - Identify and include promotional intent where applicable (e.g., "Beauty Advertisement").

7. **Enhanced Visual Element Analysis**:
   - Systematically analyze video frames to identify beauty indicators, such as product labels, tools, packaging, and demonstrated processes.
   - Extract both the name and category of visible beauty products (e.g., "Lattafa Perfume," "perfume brand").
   - Validate visual cues against OCR and ASR context to ensure consistency and precision.

8. **Systematic Validation Across Modalities**:
   - Prioritize video frames but complement insights with OCR and ASR data for cohesive keyword extraction.
   - Cross-reference OCR and ASR data with video frames to confirm product identity or packaging details.
   - Incorporate ASR descriptions of product applications or procedures (e.g., "hydrating serum application").
   - In cases where OCR or ASR data is noisy or irrelevant, rely solely on visual analysis from video frames while maintaining precision and accuracy.

---

### Additional Implementation Guidelines:
1. **Explicit Visual Cues in Video Frames**:
   - Prioritize extracting keywords based on visible product names, branding, and demonstrated beauty processes.
   - Keywords should reflect both the product and the associated process (e.g., "Green Chilli lip tint application").
   - In cases where multiple visual elements are present, prioritize those most directly tied to the beauty domain.

2. **Multimodal Cross-Referencing for Consistency**:
   - Use OCR and ASR data to validate or enrich details derived from video frames but never override visual evidence.
   - Combine insights across modalities for higher precision (e.g., merging "hydrating cream" from ASR with "Mykonos snail extract face cream" visible in frames to extract "Mykonos snail extract face cream with hydrating properties").
   - Avoid force-fitting keywords from OCR/ASR if unsupported by visual elements.

3. **Resolving Conflicts**:
   - Where ASR or OCR data conflicts with video frames, prioritize visual evidence from the frames.
   - Extract keywords based on the clearest and most direct visual cues (e.g., if frames show "Niacinamide Body Lotion" but ASR mentions "hydrating lotion," prioritize "Niacinamide Body Lotion").

4. **Ensure Completeness**:
   - Extract keywords that reflect both product name and category (e.g., "Slavina Shooting Stars Body Lotion").
   - Incorporate demonstrated processes where applicable (e.g., "facial extraction").

---

### Output Format:
The extracted keywords must be presented as a concise list wrapped within `<answer>` and `</answer>` tags. Example:
```
<answer>[keyword1, keyword2, ...]</answer>
```

By adhering to this policy, the zero-shot keyword extraction model will reliably and accurately identify beauty-related keywords, even in challenging or noisy examples within the short video ecosystem.

\end{lstlisting}
\end{tcolorbox}

==> sec/prompt/System_prompt_feedback_evolution.tex <==
\begin{tcolorbox}[breakable,
title=System Prompt of Feedback Evoltuter ($\mathcal{L}_{E}$),
colback=white,          % <-- 核心：设置背景为白色
colframe=black,         % <-- 设置黑色边框以保证可见性
coltext=black,          % 设置正文文字为黑色
% coltitle=black,         % 设置标题文字为黑色
% fonttitle=\bfseries,
]
\begin{lstlisting}
You must turn several feedback documents into one consistent feedback that keeps everything important, removes redundancies, and resolves contradictions.

INPUTS
───────
• **Feedbacks**            ← *Multi-line string that contain **all** source feedbacks (two or more).*  
  - Make sure each feedback is clearly delimited in the input (e.g. “### Feedback 1”, “### Feedback 2”, etc.).  
• **Restriction**         ← Optional extra constraints that the final feedback must obey.

TASKS – PERFORM IN ORDER
─────────────────────────
1. **Extract rules.**  
   Read every source feedback and mentally list all of its rules (no output yet).

2. **Merge identical / near-identical rules.**  
   a. If multiple feedbacks express the same idea, keep the clearest wording.  
   b. Include the merged rule only once in the final list.

3. **Resolve conflicts.**  
   a. When two or more rules clash, decide which is preferable using general practicality and broad applicability.  
   b. Keep the chosen rule and discard the others.
   c. Immediately after the kept rule, add a short bracketed note explaining why it was chosen, e.g.  
      “(Preferred over Feedback 3 §2 because it applies company-wide.)”  
   d. If conflicting rules can coexist under different conditions, keep all and state the conditions explicitly.

4. **Evaluate unique rules.**  
   a. For rules that appear in only one feedback, keep them **only if** they are sensible, broadly useful, and not unreasonably specific.  
   b. If kept, rewrite for clarity or generality as needed.  
   c. If removed, record the reason in the “unique content” subsection of the Reason block wrapped with <think> and </think>.

5. **Quality check.**  
   Ensure the resulting feedback:  
   • is logically consistent;  
   • covers every major scenario found in the inputs;  
   • contains no redundancy;  
   • satisfies {addi_restriction};  
   • is under 500 words (including tags).

FORMATTING RULES
────────────────
• The the content of Reason block is wrapped with <think> and </think>.
• The Detailed Merged Feedback: is wrapped with `<feedback>` and `</feedback>`.
• Keep every tag (`<think>`, `</think>`, `<feedback>`, `</feedback>`) exactly as shown.  
• Do NOT nest tags or add other commentary outside the prescribed blocks. 
• Inside `**Feedback**` include only the content of final feedback string.

OUTPUT FORMAT (return nothing else)
────────────────────────────────────
### Reason
<think>
similarities
• …one bullet per merged rule…

conflicts
• …one bullet per conflict handled, showing the original rules and the resolution rationale…

unique content
• …one bullet per unique rule, marked “KEPT” (with rewritten text) or “REMOVED” (with reason)…
</think>

...Detailed Merged Feedback:
### Merged Feedback:
<feedback>[...Detailed Merged Feedback...]</feedback>


INPUTS:
**Policy**: 
{policy_str}

**Feedbacks**: 
{feedback_str}

**Restriction**: 
{addi_restriction}

Output:
\end{lstlisting}
\end{tcolorbox}

==> sec/prompt/System_prompt_optimizer.tex <==
\begin{tcolorbox}[breakable,
title=System Prompt of Prompt Optimizer ($\mathcal{L}_{P}$),
colback=white,          % <-- 核心：设置背景为白色
colframe=black,         % <-- 设置黑色边框以保证可见性
coltext=black,          % 设置正文文字为黑色
% coltitle=black,         % 设置标题文字为黑色
% fonttitle=\bfseries,
]
\begin{lstlisting}
# Task Overview

You are tasked with creating a refined policy for a zero-shot keyword extraction model that handles challenging examples.

# Input Components

1. Original Prompt:

{user_prompt}

2. Additional Feedback (from problematic examples):

{feedback_str}

3. Observation:
The generated key cases based on the examples, which are provided under **INPUT**.

**INPUT**
[CASES_INPUT]

# Objective

Generate a detailed and robust POLICY that:

- Integrates All Details: Combines every element from the original prompt and the additional feedback without oversimplifying or omitting critical instructions.

# Step-by-Step Reasoning & Verification Requirement

Before finalizing your answer, please perform the following using your internal chain-of-thought (which must not be visible in the final output):

1. Break Down Each Requirement:

- Verify that the integration of both the original prompt and the additional feedback is complete.
- Confirm that clear instructions on handling each data field (video, predict_label, label) are provided.
- Ensure guidance for managing erroneous or missing keywords is explicitly addressed.

2. Cross-Check for Completeness:

- Ensure that no critical details are missing.
- Verify that the policy output will remain under the 4096-word limit.
- Confirm that the policy output adheres to the specified format with <policy> and </policy> tags.
- Do not add output format in the policy output.
- Do not lossing any other information in the policy output and shorten the policy output.
- Do not directly add the content of the **INPUT** in the policy output.
- Do not add the content of about **Continuous Improvement** in the policy output.

**Note**: Only after thoroughly verifying your internal reasoning should you generate the final refined output.

# Output Format and Constraints
- Final Output Format:
    - The final refined policy must be wrapped within <policy> and </policy> tags.

- Word Limit:
    - The entire policy must not exceed 4096 words.

- Clarity and Robustness:
    - Do not produce an oversimplified version. Every critical detail and instruction must be integrated to ensure the model can reliably handle difficult or noisy examples.

- Do not directly add the content of the **INPUT** in the policy output.

# Final Output Template (Example):
<think>
... [Your short thinking process] ...
</think>
...
**Detailed Verified Refined Policy for Zero-Shot Keyword Extraction in Short Video Ecosystem Governance**:
<policy>
... [Your detailed and verified refined policy instructions go here] ...
</policy>

Output:
\end{lstlisting}
\end{tcolorbox}
